nGraph-HE2: A High-Throughput Framework for Neural Network Inference on Encrypted Data

In previous work, Boemer et al. introduced nGraph-HE, an extension to the Intel nGraph deep learning (DL) compiler, that enables data scientists to deploy models with popular frameworks such as TensorFlow and PyTorch with minimal code changes. However, the class of supported models was limited to relatively shallow networks with polynomial activations. Here, we introduce nGraph-HE2, which extends nGraph-HE to enable privacy-preserving inference on standard, pre-trained models using their native activation functions and number fields (typically real numbers). The proposed framework leverages the CKKS scheme, whose support for real numbers is friendly to data science, and a client-aided model using a two-party approach to compute activation functions. We first present CKKS-specific optimizations, enabling a 3x-88x runtime speedup for scalar encoding, and doubling the throughput through a novel use of CKKS plaintext packing into complex numbers. Second, we optimize ciphertext-plaintext addition and multiplication, yielding 2.6x-4.2x runtime speedup. Third, we exploit two graph-level optimizations: lazy rescaling and depth-aware encoding, which allow us to significantly improve performance. Together, these optimizations enable state-of-the-art throughput of 1,998 images/s on the CryptoNets network. Using the client-aided model, we also present homomorphic evaluation of (to our knowledge) the largest network to date, namely, pre-trained MobileNetV2 models on the ImageNet dataset, with 60.4\percent/82.7\percent\ top-1/top-5 accuracy and an amortized runtime of 381 ms/image.

==> Makefile <==
all: main.pdf

# CUSTOM BUILD RULES

# In case you didn't know, '$@' is a variable holding the name of the target,
# and '$<' is a variable holding the (first) dependency of a rule.
# "raw2tex" and "dat2tex" are just placeholders for whatever custom steps
# you might have.

%.tex: %.raw
	./raw2tex $< > $@

%.tex: %.dat
	./dat2tex $< > $@

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interaction=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

main.pdf: main.tex
	rm -f main.pdf && latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -use-make main.tex

clean:
	rm -f main.bbl
	latexmk -CA

check:
	aspell --lang=en --mode=tex check abstract.tex
	aspell --lang=en --mode=tex check appendix.tex
	aspell --lang=en --mode=tex check background.tex
	aspell --lang=en --mode=tex check body.tex
	aspell --lang=en --mode=tex check extensions.tex
	aspell --lang=en --mode=tex check implementation.tex
	aspell --lang=en --mode=tex check introduction.tex
	aspell --lang=en --mode=tex check main.tex
	aspell --lang=en --mode=tex check results.tex

	# Should have ~ instead of space before any references / citations
	cat r*.tex | grep ' \\cite'
	cat r*.tex | grep ' \\ref'

.PHONY: main.pdf

